Laser excited super resolution thermal imaging for nondestructive inspection of internal defects

A photothermal super resolution technique is proposed for an improved inspection of internal defects. To evaluate the potential of the laser-based thermographic technique, an additively manufactured stainless steel specimen with closely spaced internal cavities is used. Four different experimental configurations in transmission, reflection, stepwise and continuous scanning are investigated. The applied image post-processing method is based on compressed sensing and makes use of the block sparsity from multiple measurement events. This concerted approach of experimental measurement strategy and numerical optimization enables the resolution of internal defects and outperforms conventional thermographic inspection techniques.

==> prozessdiagram.pgf.tex <==
\tikzstyle{block} = [draw, fill=white, rectangle, 
    minimum height=11mm, minimum width=16.5mm]
\tikzstyle{pic} = [inner sep=0pt,
    minimum height=18mm, minimum width=22mm]
    
\tikzstyle{picPSF} = [ inner sep=0pt,
    minimum height=14mm, minimum width=22mm]
    
\tikzstyle{picijosp} = [inner sep=0pt,
    minimum height=6mm, minimum width=22mm]
    
\tikzstyle{sum} = [draw, fill=white, circle, node distance=3cm]
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]

\newcommand\nodehspace{3cm}
\newcommand\nodehspacesmall{2.5cm}
\newcommand\nodehspacesum{2.2cm}
\newcommand\vspacesmall{1.15cm}
\newcommand\vspaceno{1.5cm}

\begin{tikzpicture}[auto , node distance=3cm,>=latex']
    \node [block, align=center](siginv) {sign \\ inversion};
    \node [block, right of=siginv,node distance=22mm] (ijosp) {IJOSP};

	\draw [draw,->, anchor=south] (siginv) -- node[name=middleijosp, anchor=north] {} (ijosp);    
    
    \node [block, right of=ijosp,node distance=\nodehspacesum] (sum) {$\sum_{N_{meas/t}}$};
    \draw [draw,->, anchor=south] (ijosp) -- node[name=summiddle, near start] {} (sum);
    
    \node [block, left of=siginv,node distance=25mm] (trans) {Tx-signal?};
    \coordinate [left of=trans, node distance=28mm] (transleft) {};
    \coordinate [left of=trans, node distance=1.3cm] (transleftarr) {};  
    \node [left of=trans, node distance=6.3cm,outer sep=0, inner sep=0] (leftend) {};
    \node [block, above of=transleft,node distance=\vspacesmall, align=center] (mt) {max.\\ thermogram};

    \coordinate [above of=mt, node distance=0.65cm] (mtabove) {};

    \coordinate [below of=trans, node distance=1.1cm] (transbelow) {};
   
    \draw [draw,->, anchor=south] (trans) -- node[name=middleyes] {yes} (siginv);
 	\coordinate [below of=middleyes, node distance=\vspaceno] (yesbelow) {};    
    
    \coordinate [above of=ijosp, node distance=1.65cm] (ijospabove) {};  
    \coordinate [below of=ijosp, node distance=21.5mm] (ijospbelow) {};   

    \coordinate [below of=middleijosp, node distance=0.8cm] (middleijospbelow) {};
    \node [ below of=middleyes, anchor=south ,node distance=11.5mm] (no) {no};
    \node [ below of=leftend, anchor=north west ,node distance=0.05cm] (cont) {\textbf{continuous:}};
    \node [ above of=leftend, anchor=north west ,node distance=2.7cm] (step) {\textbf{step:}};

    \draw [-,shorten >=0pt] (middleijospbelow) -| (trans);
    \draw [-{Circle[length=1mm]},shorten >=-8pt] (middleijospbelow) -- node {} (middleijosp);
        
    \draw[densely dashed] [draw,-, anchor=south, shorten <=0.1cm] (transleftarr) -- node {} (leftend);
    \coordinate [right of=sum, node distance=3.9cm] (rightend) {};
	\draw[densely dashed] [draw,-, anchor=south, shorten <=2.5cm] (sum) -- node {} (rightend);
    
    \draw [-,shorten >=0pt] (mt) -| node {} (transleftarr);
    \coordinate [above of=transleftarr, node distance=\vspacesmall] (mtmiddle) {};

    \draw [draw,{Circle[length=1mm]}->, shorten <=-1.25pt] (transleftarr) -- node {} (trans);
    
    %Prec:
    \node [minimum height=10mm, minimum width=23mm, right of=ijospbelow, node distance=2.65cm, inner sep=0pt] (co1) {\includegraphics[width=23mm, height=10mm]{./TikzPictures/Prec.png}};
    \node [minimum height=10mm, minimum width=23mm, above of=co1, node distance=12mm] (co1y) {};
    \node [minimum height=10mm, minimum width=23mm, right of=co1, node distance=26mm] (co1x) {};
    \draw [draw,->] (co1.south west) -- node[near end, name=xtext] {} (co1x.south west);
    \draw [draw,->] (co1.south west) -- node[near end, name=ytext] {} (co1y.south west);
    \node [ left of=ytext, anchor=north east ,node distance=-0.03cm] () {\scriptsize{$r$}};
    \node [ below of=xtext, anchor=north west ,node distance=0.15cm] () {\scriptsize{$i$}};
    \node [ above of=co1, anchor=north ,node distance=11.5mm] () {\hspace{23mm}$\hat{x}_{\text{IJOSP,\,step/cont}} \in \mathbb{R}^{N_r \times N_{meas/t}}$};
	\draw [draw,o-, shorten <=-2.5pt, shorten >=1pt] (summiddle) |- node {} (co1);
	
	%T_rec:
	\node [minimum height=7mm, minimum width=24mm, right of=sum, node distance=2.5cm, inner sep=0pt] (co2) {\input{./TikzPictures/Tijosp.pgf}};
    \node [minimum height=7mm, minimum width=24mm, above of=co2, node distance=7mm] (co2y) {};
    \node [minimum height=7mm, minimum width=24mm, right of=co2, node distance=25mm] (co2x) {};
    \draw [draw,->] (co2.south west) -- node[near end, name=xtext2] {} (co2x.south west);
    \draw [draw,->] (co2.south west) -- node[near end, name=ytext2] {} (co2y.south west);
    \node [ above of=ytext2, anchor=west, node distance=0.3cm] () {\scriptsize{$Amp.$}};
    \node [ below of=xtext2, anchor=north west ,node distance=0.15cm] () {\scriptsize{$r$}};
    \node [ above of=co2, anchor=north ,node distance=9mm] () {\hspace{13mm}$\hat{x}_{1D} \in \mathbb{R}^{N_r \times 1}$}; 
	\draw [draw,->, anchor=south, shorten >=1pt] (sum) -- node {} (co2);
	
	%PSF_step:
	\node [minimum height=7mm, minimum width=24mm, above of=ijosp,node distance=1.65cm, inner sep=0pt] (co3) {\input{./TikzPictures/PSFrec_rx.pgf}};
    \node [minimum height=7mm, minimum width=24mm, above of=co3, node distance=7mm] (co3y) {};
    \node [minimum height=7mm, minimum width=24mm, right of=co3, node distance=25mm] (co3x) {};
    \draw [draw,->] (co3.south west) -- node[near end, name=xtext3] {} (co3x.south west);
    \draw [draw,->] (co3.south west) -- node[near end, name=ytext3] {} (co3y.south west);
    \node [ above of=ytext3, anchor=west, node distance=0.3cm] () {\scriptsize{$Amp.$}};
    \node [ below of=xtext3, anchor=north west ,node distance=0.15cm] () {\scriptsize{$r$}};
    \node [ above of=co3, anchor=north ,node distance=9mm] () {\hspace{15mm}$\Phi_{\text{step}} \in  \mathbb{R}^{N_r \times 1}$};
    \draw [draw,->, anchor=south, shorten <=1pt] (co3) -- node {} (ijosp);
    
    %PSF_cont:
    \node [minimum height=10mm, minimum width=23mm,  left of=ijospbelow,node distance=17.5mm, inner sep=0pt] (co4) {\includegraphics[width=23mm, height=10mm]{./TikzPictures/PSFtxcont.png}};
    \node [minimum height=10mm, minimum width=23mm, above of=co4, node distance=12mm] (co4y) {};
    \node [minimum height=10mm, minimum width=23mm, right of=co4, node distance=26mm] (co4x) {};
    \draw [draw,->] (co4.south west) -- node[near end, name=xtext] {} (co4x.south west);
    \draw [draw,->] (co4.south west) -- node[near end, name=ytext] {} (co4y.south west);
    \node [ left of=ytext, anchor=north east ,node distance=-0.03cm] () {\scriptsize{$r$}};
    \node [ below of=xtext, anchor=north west ,node distance=0.15cm] () {\scriptsize{$t$}};
    \node [ above of=co4, anchor=north ,node distance=11.5mm] () {\hspace{5mm}$\Phi_{\text{cont}} \in \mathbb{R}^{N_r \times N_{t}}$};
	\draw [draw,->, anchor=south, shorten <=1pt] (co4) -| node {} (ijosp);   
	
	%MT:
    \node [minimum height=10mm, minimum width=23mm, right of=mtabove,node distance=30mm, inner sep=0pt] (co5) {\includegraphics[width=23mm, height=10mm]{./TikzPictures/MT.png}};
    \node [minimum height=10mm, minimum width=23mm, above of=co5, node distance=12mm] (co5y) {};
    \node [minimum height=10mm, minimum width=23mm, right of=co5, node distance=26mm] (co5x) {};
    \draw [draw,->] (co5.south west) -- node[near end, name=xtext] {} (co5x.south west);
    \draw [draw,->] (co5.south west) -- node[near end, name=ytext] {} (co5y.south west);
    \node [ left of=ytext, anchor=north east ,node distance=-0.03cm] () {\scriptsize{$r$}};
    \node [ below of=xtext, anchor=north west ,node distance=0.15cm] () {\scriptsize{$i$}};
    \node [ above of=co5, anchor=north ,node distance=11.5mm] () {\hspace{5mm}$T_{\text{step}} \in \mathbb{R}^{N_r \times N_{meas}}$};
	\draw [draw,o-, shorten <=-2.5pt] (mtmiddle) -- node {} (co5);
	
	%Tcont:
    \node [minimum height=10mm, minimum width=23mm, below of=transleft,node distance=13mm, inner sep=0pt] (co6) {\includegraphics[width=23mm, height=10mm]{./TikzPictures/Tcont.png}};
    \node [minimum height=10mm, minimum width=23mm, above of=co6, node distance=12mm] (co6y) {};
    \node [minimum height=10mm, minimum width=23mm, right of=co6, node distance=26mm] (co6x) {};
    \draw [draw,->] (co6.south west) -- node[near end, name=xtext] {} (co6x.south west);
    \draw [draw,->] (co6.south west) -- node[near end, name=ytext] {} (co6y.south west);
    \node [ left of=ytext, anchor=north east ,node distance=-0.03cm] () {\scriptsize{$r$}};
    \node [ below of=xtext, anchor=north west ,node distance=0.15cm] () {\scriptsize{$t$}};
    \node [ above of=co6, anchor=north ,node distance=13mm] () {\hspace{-0mm}$T_{\text{meas,\,cont}} \in \mathbb{R}^{N_r \times N_{t}}$};
    \draw [-,shorten <=1pt] (co6) -| (transleftarr);
    
    %Tstep
    \node [minimum height=10mm, minimum width=13mm,left of=mt,node distance=23mm, inner sep=0pt] (co72) {};
    \coordinate[below of=co72, node distance=7] (co72b) {};
    
    \node [minimum height=10mm, minimum width=13mm, left of=co72b, node distance=3mm, inner sep=0pt] (co7) {\includegraphics[width=13mm, height=10mm]{./TikzPictures/Tstep0.png}};
    \node [minimum height=10mm, minimum width=13mm, above of=co7, node distance=12mm] (co7y) {};
    \node [minimum height=10mm, minimum width=13mm, right of=co7, node distance=15mm] (co7x) {};
    \coordinate[above of=co72, node distance=7] (co72a) {};
    \node [minimum height=10mm, minimum width=13mm, right of=co72a, node distance=3mm, inner sep=0pt] (co73) {};
    \draw [draw,->] (co7.south west) -- node[near end, name=xtext] {} (co7x.south west);
    \draw [draw,->] (co7.south west) -- node[near end, name=ytext] {} (co7y.south west);
    \node [ left of=ytext, anchor=north east ,node distance=-0.03cm] () {\scriptsize{$r$}};
    \node [ below of=xtext, anchor=north west ,node distance=0.15cm] () {\scriptsize{$t$}};
    
    \node [minimum height=10mm, minimum width=13mm, above of=co7y, node distance=1.5mm] (co7ya) {};
    \node [minimum height=10mm, minimum width=13mm, above of=co73, node distance=12mm] (co73y) {};
    \draw [draw,->] (co7ya.south west) -- node[near end, name=ztext] {} (co73y.south west);
    \node [ above of=ztext, anchor=south east ,node distance=-3mm] () {\scriptsize{$i$}};
    \node [ above of=co73, anchor=north ,node distance=11mm] () {\hspace{25mm}$T_{\text{meas,\,step}} \in \mathbb{R}^{N_r \times N_{t} \times N_{meas}}$};
    \draw [draw,->, anchor=south ,shorten <=10pt] (co72) -- node {} (mt);
    \node [minimum height=10mm, minimum width=13mm,left of=co72,node distance=0mm, inner sep=0pt] (co722) {\includegraphics[width=13mm, height=10mm]{./TikzPictures/Tstep1.png}};
    \node [minimum height=10mm, minimum width=13mm, right of=co73, node distance=0mm, inner sep=0pt] (co732) {\includegraphics[width=13mm, height=10mm]{./TikzPictures/Tstep2.png}};
	
	%\path (leftend) let   \p1 = ($ (leftend) - (rightend) $),  \n1 = {veclen(\x1,\y1)} in -- (rightend) node[draw, near start] {With veclen the length is :\convertto{mm}{\n1}};
\end{tikzpicture}

==> prozessdiagram2.pgf.tex <==
\tikzstyle{block} = [draw, fill=white, rectangle, 
    minimum height=11mm, minimum width=16.5mm]
\tikzstyle{pic} = [inner sep=0pt,
    minimum height=18mm, minimum width=22mm]
    
\tikzstyle{picPSF} = [ inner sep=0pt,
    minimum height=14mm, minimum width=22mm]
    
\tikzstyle{picijosp} = [inner sep=0pt,
    minimum height=6mm, minimum width=22mm]
    
\tikzstyle{sum} = [draw, fill=white, circle, node distance=3cm]
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]

\newcommand\nodehspace{3cm}
\newcommand\nodehspacesmall{2.5cm}
\newcommand\nodehspacesum{2.2cm}
\newcommand\vspacesmall{1.15cm}
\newcommand\vspaceno{1.1cm}

\begin{tikzpicture}[auto , node distance=3cm,>=latex']
    \node [block, align=center](siginv) {sign \\ inversion};
    \node [block, right of=siginv,node distance=22mm] (ijosp) {IJOSP};

	\draw [draw,->, anchor=south] (siginv) -- node[name=middleijosp, anchor=north] {} (ijosp);    
    
    \node [block, right of=ijosp,node distance=\nodehspacesum] (sum) {$\sum_{N_{\mathrm{meas/}t}}$};
    \draw [draw,->, anchor=south] (ijosp) -- node[name=summiddle, near start] {} (sum);
    
    \node [block, left of=siginv,node distance=23mm] (trans) {Tx-signal?};
    \coordinate [left of=trans, node distance=\nodehspacesmall] (transleft) {};
    \coordinate [left of=trans, node distance=1.3cm] (transleftarr) {};  
    \node [left of=trans, node distance=6.3cm,outer sep=0, inner sep=0] (leftend) {};
    \node [block, above of=transleft,node distance=\vspacesmall, align=center] (mt) {max.\\ thermogram};

    \coordinate [above of=mt, node distance=0.5cm] (mtabove) {};

    \coordinate [below of=trans, node distance=1.1cm] (transbelow) {};
   
    \draw [draw,->, anchor=south] (trans) -- node[name=middleyes] {yes} (siginv);
 	\coordinate [below of=middleyes, node distance=\vspaceno] (yesbelow) {};    
    
    \coordinate [above of=ijosp, node distance=1.65cm] (ijospabove) {};  
    \coordinate [below of=ijosp, node distance=1.8cm] (ijospbelow) {};   

    \coordinate [below of=middleijosp, node distance=0.6cm] (middleijospbelow) {};
    \node [ below of=middleyes, anchor=south ,node distance=0.95cm] (no) {no};
    \node [ below of=leftend, anchor=north west ,node distance=0.05cm] (cont) {\textbf{continuous:}};
    \node [ above of=leftend, anchor=north west ,node distance=2.7cm] (step) {\textbf{step:}};

    \draw [-,shorten >=0pt] (middleijospbelow) -| (trans);
    \draw [-{Circle[length=1mm]},shorten >=-7.75pt] (middleijospbelow) -- node {} (middleijosp);
        
    \draw[densely dashed] [draw,-, anchor=south, shorten <=0.1cm] (transleftarr) -- node {} (leftend);
    \coordinate [right of=sum, node distance=3.9cm] (rightend) {};
	\draw[densely dashed] [draw,-, anchor=south, shorten <=2.5cm] (sum) -- node {} (rightend);
    
    \draw [-,shorten >=0pt] (mt) -| node {} (transleftarr);
    \coordinate [above of=transleftarr, node distance=\vspacesmall] (mtmiddle) {};

    \draw [draw,{Circle[length=1mm]}->, shorten <=-1.25pt] (transleftarr) -- node {} (trans);
    
    %Prec:
    \node [minimum height=7mm, minimum width=20mm, right of=ijospbelow, node distance=2.5cm, inner sep=0pt] (co1) {\includegraphics[width=20mm, height=7mm]{./TikzPictures/Prec.png}};
    \node [minimum height=7mm, minimum width=20mm, above of=co1, node distance=9mm] (co1y) {};
    \node [minimum height=7mm, minimum width=20mm, right of=co1, node distance=23mm] (co1x) {};
    \draw [draw,->] (co1.south west) -- node[near end, name=xtext] {} (co1x.south west);
    \draw [draw,->] (co1.south west) -- node[near end, name=ytext] {} (co1y.south west);
    \node [ left of=ytext, anchor=north east ,node distance=-0.03cm] () {\scriptsize{$r$}};
    \node [ below of=xtext, anchor=north west ,node distance=0.15cm] () {\scriptsize{$i$}};
    \node [ above of=co1, anchor=north ,node distance=10mm] () {\hspace{23mm}$\hat{x}_{\mathrm{IJOSP,\,step/cont}} \in \mathbb{R}^{N_r \times N_{\mathrm{meas/}t}}$};
	\draw [draw,o-, shorten <=-2.5pt, shorten >=1pt] (summiddle) |- node {} (co1);
	
	%T_rec:
	\node [minimum height=7mm, minimum width=24mm, right of=sum, node distance=2.5cm, inner sep=0pt] (co2) {\input{./TikzPictures/Tijosp.pgf}};
    \node [minimum height=7mm, minimum width=24mm, above of=co2, node distance=7mm] (co2y) {};
    \node [minimum height=7mm, minimum width=24mm, right of=co2, node distance=25mm] (co2x) {};
    \draw [draw,->] (co2.south west) -- node[near end, name=xtext2] {} (co2x.south west);
    \draw [draw,->] (co2.south west) -- node[near end, name=ytext2] {} (co2y.south west);
    \node [ above of=ytext2, anchor=west, node distance=0.3cm] () {\scriptsize{$Amp.$}};
    \node [ below of=xtext2, anchor=north west ,node distance=0.15cm] () {\scriptsize{$r$}};
    \node [ above of=co2, anchor=north ,node distance=9mm] () {\hspace{13mm}$\hat{x} \in \mathbb{R}^{N_r \times 1}$}; 
	\draw [draw,->, anchor=south, shorten >=1pt] (sum) -- node {} (co2);
	
	%PSF_step:
	\node [minimum height=7mm, minimum width=24mm, above of=ijosp,node distance=1.65cm, inner sep=0pt] (co3) {\input{./TikzPictures/PSFrec_rx.pgf}};
    \node [minimum height=7mm, minimum width=24mm, above of=co3, node distance=7mm] (co3y) {};
    \node [minimum height=7mm, minimum width=24mm, right of=co3, node distance=25mm] (co3x) {};
    \draw [draw,->] (co3.south west) -- node[near end, name=xtext3] {} (co3x.south west);
    \draw [draw,->] (co3.south west) -- node[near end, name=ytext3] {} (co3y.south west);
    \node [ above of=ytext3, anchor=west, node distance=0.3cm] () {\scriptsize{$Amp.$}};
    \node [ below of=xtext3, anchor=north west ,node distance=0.15cm] () {\scriptsize{$r$}};
    \node [ above of=co3, anchor=north ,node distance=9mm] () {\hspace{15mm}$\Phi_{\mathrm{step}} \in  \mathbb{R}^{N_r \times 1}$};
    \draw [draw,->, anchor=south, shorten <=1pt] (co3) -- node {} (ijosp);
    
    %PSF_cont:
    \node [minimum height=7mm, minimum width=20mm,  left of=ijospbelow,node distance=1.6cm, inner sep=0pt] (co4) {\includegraphics[width=20mm, height=7mm]{./TikzPictures/PSFtxcont.png}};
    \node [minimum height=7mm, minimum width=20mm, above of=co4, node distance=9mm] (co4y) {};
    \node [minimum height=7mm, minimum width=20mm, right of=co4, node distance=23mm] (co4x) {};
    \draw [draw,->] (co4.south west) -- node[near end, name=xtext] {} (co4x.south west);
    \draw [draw,->] (co4.south west) -- node[near end, name=ytext] {} (co4y.south west);
    \node [ left of=ytext, anchor=north east ,node distance=-0.03cm] () {\scriptsize{$r$}};
    \node [ below of=xtext, anchor=north west ,node distance=0.15cm] () {\scriptsize{$t$}};
    \node [ above of=co4, anchor=north ,node distance=10mm] () {\hspace{5mm}$\Phi_{\mathrm{cont}} \in \mathbb{R}^{N_r \times N_{t}}$};
	\draw [draw,->, anchor=south, shorten <=1pt] (co4) -| node {} (ijosp);   
	
	%MT:
    \node [minimum height=7mm, minimum width=20mm, right of=mtabove,node distance=2.6cm, inner sep=0pt] (co5) {\includegraphics[width=20mm, height=7mm]{./TikzPictures/MT.png}};
    \node [minimum height=7mm, minimum width=20mm, above of=co5, node distance=9mm] (co5y) {};
    \node [minimum height=7mm, minimum width=20mm, right of=co5, node distance=23mm] (co5x) {};
    \draw [draw,->] (co5.south west) -- node[near end, name=xtext] {} (co5x.south west);
    \draw [draw,->] (co5.south west) -- node[near end, name=ytext] {} (co5y.south west);
    \node [ left of=ytext, anchor=north east ,node distance=-0.03cm] () {\scriptsize{$r$}};
    \node [ below of=xtext, anchor=north west ,node distance=0.15cm] () {\scriptsize{$i$}};
    \node [ above of=co5, anchor=north ,node distance=10mm] () {\hspace{5mm}$T_{\mathrm{step}} \in \mathbb{R}^{N_r \times N_{\mathrm{meas}}}$};
	\draw [draw,o-, shorten <=-2.5pt] (mtmiddle) -- node {} (co5);
	
	%Tcont:
    \node [minimum height=7mm, minimum width=20mm, below of=transleft,node distance=\vspacesmall, inner sep=0pt] (co6) {\includegraphics[width=20mm, height=7mm]{./TikzPictures/Tcont.png}};
    \node [minimum height=7mm, minimum width=20mm, above of=co6, node distance=9mm] (co6y) {};
    \node [minimum height=7mm, minimum width=20mm, right of=co6, node distance=23mm] (co6x) {};
    \draw [draw,->] (co6.south west) -- node[near end, name=xtext] {} (co6x.south west);
    \draw [draw,->] (co6.south west) -- node[near end, name=ytext] {} (co6y.south west);
    \node [ left of=ytext, anchor=north east ,node distance=-0.03cm] () {\scriptsize{$r$}};
    \node [ below of=xtext, anchor=north west ,node distance=0.15cm] () {\scriptsize{$t$}};
    \node [ above of=co6, anchor=north ,node distance=11mm] () {\hspace{-5mm}$T_{\mathrm{meas,\,cont}} \in \mathbb{R}^{N_r \times N_{t}}$};
    \draw [-,shorten <=1pt] (co6) -| (transleftarr);
    
    %Tstep
    \node [minimum height=10mm, minimum width=13mm,left of=mt,node distance=23mm, inner sep=0pt] (co72) {};
    \coordinate[below of=co72, node distance=7] (co72b) {};
    
    \node [minimum height=10mm, minimum width=13mm, left of=co72b, node distance=3mm, inner sep=0pt] (co7) {\includegraphics[width=13mm, height=10mm]{./TikzPictures/Tstep0.png}};
    \node [minimum height=10mm, minimum width=13mm, above of=co7, node distance=12mm] (co7y) {};
    \node [minimum height=10mm, minimum width=13mm, right of=co7, node distance=15mm] (co7x) {};
    \coordinate[above of=co72, node distance=7] (co72a) {};
    \node [minimum height=10mm, minimum width=13mm, right of=co72a, node distance=3mm, inner sep=0pt] (co73) {};
    \draw [draw,->] (co7.south west) -- node[near end, name=xtext] {} (co7x.south west);
    \draw [draw,->] (co7.south west) -- node[near end, name=ytext] {} (co7y.south west);
    \node [ left of=ytext, anchor=north east ,node distance=-0.03cm] () {\scriptsize{$r$}};
    \node [ below of=xtext, anchor=north west ,node distance=0.15cm] () {\scriptsize{$t$}};
    
    \node [minimum height=10mm, minimum width=13mm, above of=co7y, node distance=1.5mm] (co7ya) {};
    \node [minimum height=10mm, minimum width=13mm, above of=co73, node distance=12mm] (co73y) {};
    \draw [draw,->] (co7ya.south west) -- node[near end, name=ztext] {} (co73y.south west);
    \node [ above of=ztext, anchor=south east ,node distance=-3mm] () {\scriptsize{$i$}};
    \node [ above of=co73, anchor=north ,node distance=11mm] () {\hspace{23mm}$T_{\mathrm{meas,\,step}} \in \mathbb{R}^{N_r \times N_{t} \times N_{\mathrm{meas}}}$};
    \draw [draw,->, anchor=south ,shorten <=10pt] (co72) -- node {} (mt);
    \node [minimum height=10mm, minimum width=13mm,left of=co72,node distance=0mm, inner sep=0pt] (co722) {\includegraphics[width=13mm, height=10mm]{./TikzPictures/Tstep1.png}};
    \node [minimum height=10mm, minimum width=13mm, right of=co73, node distance=0mm, inner sep=0pt] (co732) {\includegraphics[width=13mm, height=10mm]{./TikzPictures/Tstep2.png}};
	
	%\path (leftend) let   \p1 = ($ (leftend) - (rightend) $),  \n1 = {veclen(\x1,\y1)} in -- (rightend) node[draw, near start] {With veclen the length is :\convertto{mm}{\n1}};
\end{tikzpicture}
